Practical Byte-Granular Memory Blacklisting using Califorms

Recent rapid strides in memory safety tools and hardware have improved software quality and security. While coarse-grained memory safety has improved, achieving memory safety at the granularity of individual objects remains a challenge due to high performance overheads which can be between ~1.7x-2.2x. In this paper, we present a novel idea called Califorms, and associated program observations, to obtain a low overhead security solution for practical, byte-granular memory safety. The idea we build on is called memory blacklisting, which prohibits a program from accessing certain memory regions based on program semantics. State of the art hardware-supported memory blacklisting while much faster than software blacklisting creates memory fragmentation (of the order of few bytes) for each use of the blacklisted location. In this paper, we observe that metadata used for blacklisting can be stored in dead spaces in a program's data memory and that this metadata can be integrated into microarchitecture by changing the cache line format. Using these observations, Califorms based system proposed in this paper reduces the performance overheads of memory safety to ~1.02x-1.16x while providing byte-granular protection and maintaining very low hardware overheads. The low overhead offered by Califorms enables always on, memory safety for small and large objects alike, and the fundamental idea of storing metadata in empty spaces, and microarchitecture can be used for other security and performance applications.

==> securitypolicy.tex <==
\section{Security Policy}\label{sec:securitypolicy}
\FIXME{Merge in the Software Design section}

\subsection{Overview}

This section describes our security mechanism which is a software defined policy based on \Propname{}s.
We take advantage of the fine-grained nature of \Propname{}s to embed \bytename{}s (into padding bytes) within objects in user programs.
\begin{comment}
This allows us to catch potentially anomalous accesses targeted on them.
For example, an attacker may try to influence the values of adjacent fields to alter program behaviour, or even potentially make the program reinterpret a chosen memory location as an object of some other, attacker intended type.

While this mechanism already offers a certain level of protection against attacks that exploit intra-object overflows, we further enhance security by randomly introducing more \bytename{}s within the objects, by statically altering their type layouts.
This makes it extremely difficult for the attacker to avoid running into \bytename{}s when mounting his/her attack, now that the data layout of the program is hidden.
Varying the number of \bytename{}s that we introduce into the type layouts allows us to tradeoff between security and performance.
More the number of \bytename{}s we add, more difficult it gets for an adversary to avoid accessing them.
This comes with the cost of reduced effective cache capacity and thus decreased performance, as we have seen in \refsec{sec:motivation}.

\end{comment}
We describe the invariants pertaining to creation, deletion and access of \bytename{}s that we enforce.
We define the creation and deletion invariants to ensure that,
within any allocated regions of memory, only the bytes which are legitimately (and intendedly) used by the program do not have \bytename{}s (\ie{}all the padding bytes remain as \bytename{}s).
The access invariants define what actions on \bytename{}s are (dis)allowed. %
By definition, the locations of \bytename{}s are never meant to be used in a sane manner by the program.

\subsection{Creation and Deletion Invariants}\label{subsec:creation}

\begin{comment}
In this subsection we discuss how we enforce the invariants upon memory allocation and deallocation in stack and heap regions.
We can think of two approaches: unallocated memory has no \bytename{}s, we set them (to padding locations) upon allocation and unset them upon deallocation; unallocated memory is filled with \bytename{}s, we unset them (from legitimate data locations) upon allocation and set them upon deallocation.
We opt for the latter since it offers higher security guarantees.

\fakeitem\textbf{Stack and globals.}
The \texttt{data} and \texttt{bss} segments are filled with \bytename{}s when it is allocated upon thread (process) creation.
For the stack, we instrument function prologues to hook into allocations of composite types (\eg{}\texttt{struct} instances), and execute \texttt{\INSTNAME{}} instructions to unset unnecessary \bytename{}s according to its type layout information.
We also keep track of these allocations to later set the \bytename{}s to the stack upon deallocation at function epilogues.
Similarly, for \texttt{data} and \texttt{bss} segments we unset the \bytename{}s once we enter the \texttt{main} function.
In order to ensure that the unallocated stack region is filled with \bytename{}s, inside the function epilogue we execute \texttt{\INSTNAME{}} instructions to fill the stack frame that has been used with \bytename{}s.

\fakeitem\textbf{Heap.}
Our design ensures that all newly allocated memory on heap is filled with \bytename{}s (using copy-on-write of a page filled with \bytename{}s).
We instrument all heap allocations to ensure that \bytename{}s are in all the padding regions.
We do so by associating every heap allocation with type information using our compiler pass and passing on this information to the runtime.
At runtime, our instrumented hooks at the allocation sites execute \texttt{\INSTNAME{}} instructions to unset \bytename{}s as necessary.
Our runtime also keeps track of the types and sizes of allocations to enable us to handle deallocations properly.
We instrument all \texttt{free} calls where we perform similar operations to set the \bytename{}s.
\end{comment}

In this subsection we discuss how we enforce the invariants upon memory allocation and deallocation in stack and heap regions.
The goal is to set \bytename{}s upon allocation and unset them upon deallocation.

\fakeitem\textbf{Stack and Globals.}
For the stack, we instrument function prologues to hook into allocations of composite types (\eg{}\texttt{struct} instances), and execute \texttt{\INSTNAME{}} instructions to set necessary \bytename{}s according to its type layout information.
We also keep track of these allocations to later unset the \bytename{}s to the stack upon deallocation at function epilogues.
Similarly for \texttt{data} and \texttt{bss} segments we set the \bytename{}s once we enter the \texttt{main} function.
Inside the function epilogue we execute \texttt{\INSTNAME{}} instructions to unset the unnecessary \bytename{}s from the stack frame that has been used.

\fakeitem\textbf{Heap.}
We instrument all heap allocations to ensure that \bytename{}s are in all the padding regions.
We do so by associating every heap allocation with type information using our compiler pass and passing on this information to the runtime.
At runtime, our instrumented hooks at the allocation sites execute \texttt{\INSTNAME{}} instructions to set \bytename{}s as necessary.
Our runtime also keeps track of the types and sizes of allocations to enable us to handle deallocations properly.
We instrument all \texttt{free} calls where we perform similar operations to unset the \bytename{}s.

\subsection{Access Invariants}\label{subsec:access}

In line with typical blacklisting techniques, we make the \bytename{}s inaccessible with regular loads and stores.
So, consider a class as follows:

\mint[style=bw,fontsize=\small,]{cpp}|class C { char c; int i; };|
\noindent
wherein \Propname{}s would generally insert \bytename{}s between the two elements.
Hence, the compiler will have to issue precise load and/or store instructions in accordance with the widths of the elements being accessed.
Hence, in our example, \texttt{c} has to be read with a 1B load, whereas \texttt{i} needs a separate precise 4B load.
Typically, we have found that modern compilers do indeed follow this rule.

Additionally, for the sake of usability and backwards compatibility, we
have to accommodate copying operations of the nature of \texttt{memcpy}.
For example, a simple \texttt{struct} to \texttt{struct} assignment
could trigger this behavior, thus leading to a potential breakdown of
\propname{}ed software. Hence, in order to maintain usability, we
allow whitelisting functionality to suppress the exceptions.
This is done by issuing a privileged store instruction to modify the
value of exception mask registers before entering and after exiting the
according piece of code. We discuss the implications of this design
choice in \refsec{sec:discussion}.

\begin{comment}
\subsection{Access and Communication Invariants}\label{subsec:accessandcommunication}

Enforcement of the access and communication invariants is accomplished by the hardware that monitors the access and operation on the \bytename{}s.
The goal of the mechanisms is to throw a privileged exception when one of the following conditions are met: (1) a \bytename{} is overwritten by a non-\bytename{} or (2) a \bytename{} is used as an argument of one of the following instructions, conditional branch, system call or pointer dereference.

The first condition might be a case where an adversary gained control of the program and is trying to unset the \bytename{}s from the program.
Therefore, we thrown an exception whenever we detect this event.
However one problem with this policy is that it might introduce false positives when the program relies on a custom memory allocator.
A custom allocator may reuse the allocated region without actually calling \texttt{free}.
This means that a memory region can be reused by a different type of object, where for instance the original struct contains a \bytename{} but the corresponding byte might not be a \bytename{} for the new struct.
In such case a \bytename{} may be overwritten.
We do not handle this case where \FIXME{...}

The operations of the second condition require the values to be initialized and thus we throw an exception when a \bytename{} is used\Cite{Bruening:2011wt,Seward:2005vp,Stepanov:2015ua}.
Detection requires some effort since it requires propagating the \bytename{} information to successive instructions which may or may not legitimately use the \bytename{}.
We propose two solutions with different accuracy levels and implementation complexities: sink control method and the source control method.

\subsubsection{Sink control.}

A straightforward mechanism is to accurately propagate (as much as possible) the \bytename{} on use (such as copying) and throw an exception at the sink when certain prohibited operations take place on a \bytename{}.
This algorithm is similar to the ones used in Dr.\ Memory\Cite{Bruening:2011wt}, Memcheck\Cite{Seward:2005vp} and MemorySanitizer\Cite{Stepanov:2015ua}, except that we implement the policy in hardware and also at a byte-granularity (as opposed to bit-granularity).
In order to propagate the \bytename{} information through instructions, we expand the physical register file by one bit per byte (\ie{}additional eight bits is required for a 64-bit register) to indicate whether the byte is a \bytename{} or not.
When we load \bytename{}s into the register, the corresponding bits are set.
The bits are propagated to destination registers in hardware according to the rules described in the literature\Cite{Stepanov:2015ua}.

\subsubsection{Source control.}

\newlength{\fancyvrbtopsep}
\newlength{\fancyvrbpartopsep}
\setlength{\fancyvrbtopsep}{1pt}
\setlength{\fancyvrbpartopsep}{0pt}
\makeatletter
\FV@AddToHook{\FV@ListParameterHook}{\topsep=\fancyvrbtopsep\partopsep=\fancyvrbpartopsep}
\makeatother
Another idea is to generate code which does not touch the \bytename{}s.
Consider a class like this:
\mint[style=bw,fontsize=\small,]{cpp}|class C { char c; int i; };|
\noindent
the compiler may generate a copy constructor with an eight byte load instruction which reads the value of both members including the paddings --- which are \bytename{}s --- between the two member variables.
Instead, we emit two load instructions (a single byte load and a four byte load) to avoid reading the \bytename{}s.
This way we do not need to propagate the information to further instructions because \bytename{}s are never read into the register file.

However, there are exceptions.
One notable case is \texttt{memcpy} (\eg{} copying a \texttt{struct} including its paddings) and similar library functions.
Since the compiler is not always able to detect the type information of the underlying object being copied, we cannot rely on the compiler to handle these functions.
Therefore we rely on the \textit{whitelisting} functionality to suppress the exceptions.
This is done by hooking the calls and issuing a privileged store instruction to modify the value of exception mask registers when entering/exiting the function.

\subsubsection{Hardware-only heuristic.}

We consider any operation on a \bytename{} to be malicious if it overwrites the \bytename{} within the register file.
In other words, reading a \bytename{} is allowed, and any successive operations which move the \bytename{} (\eg{}store or shift) are also allowed, but any other operations which modify the \bytename{} such as an arithmetic operation is prohibited.
For instance if a \bytename{} is being read and then written to memory, we consider it as a legitimate copy.
\end{comment}



